Risk-Averse Offline Reinforcement Learning

Training Reinforcement Learning (RL) agents in high-stakes applications might be too prohibitive due to the risk associated to exploration. Thus, the agent can only use data previously collected by safe policies. While previous work considers optimizing the average performance using offline data, we focus on optimizing a risk-averse criteria, namely the CVaR. In particular, we present the Offline Risk-Averse Actor-Critic (O-RAAC), a model-free RL algorithm that is able to learn risk-averse policies in a fully offline setting. We show that O-RAAC learns policies with higher CVaR than risk-neutral approaches in different robot control tasks. Furthermore, considering risk-averse criteria guarantees distributional robustness of the average performance with respect to particular distribution shifts. We demonstrate empirically that in the presence of natural distribution-shifts, O-RAAC learns policies with good average performance.

==> sections/old_results-expert.tex <==
\begin{table*}[t]
    \centering
    % \vspace{-1em}
    \caption { Performance of \alg, O-WCPG, O-D4PG, and RAAC on offline (E)-MuJoCo data sets. In all environments, \alg has a higher CVaR and, in environments that terminate, a longer duration than the benchmarks.
    When no VAE component is used, RAAC performs poorly.\label{table:offline-expert}}
    
\begin{tabular}{@{}ccccccc@{}}
    \toprule
    &  \textbf{Algorithm}  & \textbf{\alg} & O-WCPG & O-D4PG & RAAC \\ \midrule
    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\small{half}}}} 
    &$\text{CVaR}_{0.1}$ of Returns & \textbf{595.3  $\pm$ 191.0} & 248.4  $\pm$ 232.3 & \textbf{555.8  $\pm$ 263.2} & 2.74 $\pm$ 12.8 \\
    & Average of Returns & \textbf{1180.4  $\pm$ 77.8}  & 905.0  $\pm$ 107.2  & \textbf{1099.8  $\pm$ 152.7}  & 29.8 $\pm$ 3.0 \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{walker}}}} 
      & $\text{CVaR}_{0.1}$ of Returns& \textbf{1171.8  $\pm$ 71.3} & 361.8  $\pm$ 32.5 & 772.5  $\pm$ 54.7 & 53.9  $\pm$ 2.0 \\
    & Episode Length & \textbf{431.8  $\pm$ 11.0} & 301.4  $\pm$ 31.1 & \textbf{405.4  $\pm$ 12.2} &  195.5  $\pm$ 6.1 \\
    & Average of Duration & \textbf{2005.8  $\pm$ 56.4} & 1372.4  $\pm$ 160.1 & 1869.9  $\pm$ 62.8 & 82.9  $\pm$ 6.4 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{hopper}}}} 
    & $\text{CVaR}_{0.1}$ of Returns & \textbf{979.5  $\pm$ 27.7} & 720.0  $\pm$ 33.8 & 606.4  $\pm$ 31.4 & 473.84 $\pm$ 0.1 \\
    & Episode Duration & \textbf{463.5  $\pm$ 6.5} & 301.2  $\pm$ 0.6 & 267.7  $\pm$ 2.5 &  500 $\pm$ 0 \\

    & Average of Returns & \textbf{1384.5  $\pm$ 33.11} & 897.6  $\pm$ 12.1 & 783.1  $\pm$ 18.2 & 474.75 $\pm$ 0.1 \\
   \bottomrule
    \end{tabular}
    % \vspace{-2em}
\end{table*}
    
    
    
% \begin{table*}[t]
%     \centering
%     \caption { \label{table:offline-expert}}
% \begin{tabular}{@{}ccccccc@{}}
%     \toprule
%     &  \textbf{Algorithm}  & \textbf{\alg}-0.1 & \textbf{\alg}-0.25 & O-WCPG-0.1 & O-D4PG & RAAC \\ \midrule
%     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\small{half}}}} 
%     & Expected Value & \textbf{1180.4  $\pm$ 77.8}  & \textbf{1114.9  $\pm$ 139.2}  & 905.0  $\pm$ 107.2  & \textbf{1099.8  $\pm$ 152.7}  & 29.8 $\pm$ 3.0 \\
%     & CVaR-$0.1$ & \textbf{595.3  $\pm$ 191.0} & \textbf{483.5  $\pm$ 217.9} & 248.4  $\pm$ 232.3 & \textbf{555.8  $\pm$ 263.2} & 2.74 
%     $\pm$ 12.8 \\
%     %  & Steps & 200    &  200   &  200   &  200   \\
%     \midrule
%   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{walker}}}} 
%     & Expected Value & \textbf{2005.8  $\pm$ 56.4} & 1867.7  $\pm$ 62.9 & 1372.4  $\pm$ 160.1 & 1869.9  $\pm$ 62.8 & \\
%     & CVaR-$0.1$ & \textbf{1171.8  $\pm$ 71.3} & 815.0  $\pm$ 140.1 & 361.8  $\pm$ 32.5 & 772.5  $\pm$ 54.7 \\
%     & Episode Length & \textbf{431.8  $\pm$ 11.0} & \textbf{437.4  $\pm$ 9.3} & 301.4  $\pm$ 31.1 & 405.4  $\pm$ 12.2 &  \\
%     \midrule
%     \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{hopper}}}} 
%     & Expected Value & \textbf{1384.5  $\pm$ 33.11} & \textbf{1384.3  $\pm$ 21.4} & 897.6  $\pm$ 12.1 & 783.1  $\pm$ 18.2 & 474.75 $\pm$ 0.1 \\
%     & CVaR-$0.1$ & 979.5  $\pm$ 27.7 & \textbf{1073.0  $\pm$ 33.5} & 720.0  $\pm$ 33.8 & 606.4  $\pm$ 31.4 & 473.84 $\pm$ 0.1 \\
%     & Episode Length & \textbf{463.5  $\pm$ 6.5} & \textbf{443.3  $\pm$ 8.9} & 301.2  $\pm$ 0.6 & 267.7  $\pm$ 2.5 &  500 $\pm$ 0 \\
%   \bottomrule
%     \end{tabular}
%     % \vspace{-1mm}
% \end{table*}

==> sections/old_results-medium.tex <==
\begin{table*}[t]
    \centering
    \caption{Performance  \alg, O-WCPG, O-D4PG, and RAAC on offline MuJoCo data sets. The top sub-table shows the medium (M) environments whereas the bottom sub-table the expert (E) environments.
    In all environments, \alg has a higher CVaR than benchmarks. 
    In environments that terminate, \alg has a longer duration too. 
    Finally, \alg also has better or equivalent risk-neutral performance than benchmarks. 
    As an ablation, RAAC (without the VAE component) performs poorly in the offline setting.
    \label{table:offline-medium}}
\begin{tabular}{@{}ccccccc@{}}
    \toprule
    Env &  Criterion  & \textbf{\alg} & O-WCPG & O-D4PG & RAAC  \\ \midrule
    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{214.1 $\pm$ 35.9}  & 75.9 $\pm$ 14.3  & 66.0 $\pm$ 34.4 & -54.9  $\pm$ 0.9 \\
    & Average  Returns  & \textbf{330.6 $\pm$ 30.4}  & \textbf{316.1 $\pm$ 23.3}  & \textbf{340.6 $\pm$ 20.0}  & -51.6  $\pm$ 0.3 \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{750.5  $\pm$ 153.5} & -15.0  $\pm$ 40.7 & 30.6  $\pm$ 28.8 & 54.7  $\pm$ 2.0  \\
    & Episode Duration &  \textbf{397.4  $\pm$ 18.5}  & 184.9  $\pm$ 12.1 & 248.8  $\pm$ 8.9 & 199.8  $\pm$ 6.5 \\
    & Average  Returns  & \textbf{1282.4  $\pm$ 19.3} & 283.3  $\pm$ 36.7 & 307.7  $\pm$ 19.9 & 91.7  $\pm$ 8.9 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{1416.1  $\pm$ 28.1} & -87.1  $\pm$ 24.5 & 1007.5  $\pm$ 28.2 & 71.3  $\pm$ 23.2 \\
    & Episode Duration &  \textbf{499.3  $\pm$ 1.2} & 99.3  $\pm$ 0.1 & 358.3  $\pm$ 3.1 & 146.1  $\pm$ 4.0\\
    & Average  Returns  & \textbf{1482.2  $\pm$ 4.3} & 68.5  $\pm$ 7.6 & 1098.0  $\pm$ 10.6 & 112.8  $\pm$ 4.6\\
    \midrule 
    \midrule
    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-E}}}} 
    &$\text{CVaR}_{0.1}$  Returns & \textbf{595.3  $\pm$ 191.0} & 248.4  $\pm$ 232.3 & \textbf{555.8  $\pm$ 263.2} & 2.74 $\pm$ 12.8 \\
    & Average  Returns & \textbf{1180.4  $\pm$ 77.8}  &  \textbf{905.0  $\pm$ 107.2}  & \textbf{1099.8  $\pm$ 152.7}  & 29.8 $\pm$ 3.0 \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-E}}}} 
      & $\text{CVaR}_{0.1}$  Returns& \textbf{1171.8  $\pm$ 71.3} & 361.8  $\pm$ 32.5 & 772.5  $\pm$ 54.7 & 53.9  $\pm$ 2.0 \\
    & Episode Duration & \textbf{431.8  $\pm$ 11.0} & 301.4  $\pm$ 31.1 & \textbf{405.4  $\pm$ 12.2} &  195.5  $\pm$ 6.1 \\
    & Average  Returns & \textbf{2005.8  $\pm$ 56.4} & 1372.4  $\pm$ 160.1 & 1869.9  $\pm$ 62.8 & 82.9  $\pm$ 6.4 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-E}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{979.5  $\pm$ 27.7} & 720.0  $\pm$ 33.8 & 606.4  $\pm$ 31.4 & 473.84 $\pm$ 0.1 \\
    & Episode Duration & \textbf{463.5  $\pm$ 6.5} & 301.2  $\pm$ 0.6 & 267.7  $\pm$ 2.5 &  500 $\pm$ 0 \\

    & Average  Returns & \textbf{1384.5  $\pm$ 33.11} & 897.6  $\pm$ 12.1 & 783.1  $\pm$ 18.2 & 474.75 $\pm$ 0.1 \\
   \bottomrule
    \end{tabular}
    % \vspace{-1mm}
\end{table*}


% \begin{table*}[t]
%     \centering
%     \caption {\label{table:offline-medium}}
% \begin{tabular}{@{}ccccccc@{}}
%     \toprule
%     &  \textbf{Algorithm}  & \textbf{\alg-0.1} & \textbf{\alg-0.25} & O-WCPG-0.1 & O-D4PG & RAAC  \\ \midrule
%     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\small{half}}}} 
%     & Expected Value & \textbf{330.6 $\pm$ 30.4}  & \textbf{321.2 $\pm$ 17.0}  & \textbf{316.1 $\pm$ 23.3}  & \textbf{340.6 $\pm$ 20.0}  & -51.6  $\pm$ 0.3 \\
%     & CVaR-$0.1$ & \textbf{214.1 $\pm$ 35.9}  & \textbf{223.1 $\pm$ 44.8}  & 75.9 $\pm$ 14.3  & 66.0 $\pm$ 34.4 & -54.9  $\pm$ 0.9 \\
%     \midrule
%   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{walker}}}} 
%     & Expected Value & \textbf{1282.4  $\pm$ 19.3} & \textbf{1261.7  $\pm$ 65.7} & 283.3  $\pm$ 36.7 & 307.7  $\pm$ 19.9 \\
%     & CVaR-$0.1$ & \textbf{750.5  $\pm$ 153.5} & 405.5  $\pm$ 118.4 & -15.0  $\pm$ 40.7 & 30.6  $\pm$ 28.8 \\
%     & Steps &  397.4  $\pm$ 18.5 & \textbf{456.1  $\pm$ 15.1} & 184.9  $\pm$ 12.1 & 248.8  $\pm$ 8.9 &\\
%     \midrule
%     \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{hopper}}}} 
%     & Expected Value & \textbf{1482.2  $\pm$ 4.3} & 1293.7  $\pm$ 24.5 & 68.5  $\pm$ 7.6 & 1098.0  $\pm$ 10.6 & 112.8  $\pm$ 4.6\\
%     & CVaR-$0.1$ & \textbf{1416.1  $\pm$ 28.1} & 1085.7  $\pm$ 18.8 & -87.1  $\pm$ 24.5 & 1007.5  $\pm$ 28.2 & 71.3  $\pm$ 23.2 \\
%      & Steps &  \textbf{499.3  $\pm$ 1.2} & 404.0  $\pm$ 7.1 & 99.3  $\pm$ 0.1 & 358.3  $\pm$ 3.1 & 146.1  $\pm$ 4.0\\
%   \bottomrule
%     \end{tabular}
%     % \vspace{-1mm}
% \end{table*}



==> sections/results-ablated-expert.tex <==
\begin{table*}[t]
    \centering
    \caption { \label{table:offline-ablated-expert}}
\begin{tabular}{@{}ccccccc@{}}
        \toprule
        &  \textbf{Algorithm}  & \textbf{\alg}-0.1  \\ \midrule
        \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\small{half}}}} 
        & Expected Value & 29.79  $\pm$ 3.03 & \\
        & CVaR-$0.1$ & 2.74  $\pm$ 12.75 & \\
        %  & Steps & 200    &  200   &  200   &  200   \\
        \midrule
       \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{walker}}}} 
        & Expected Value & 82.88  $\pm$ 6.37 & \\
        & CVaR-$0.1$ & 53.86  $\pm$ 1.95 & \\
        & Episode Length 195.45  $\pm$ 6.05 &    \\
        \midrule
        \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{hopper}}}} 
        & Expected Value & 474.75  $\pm$ 0.13 & &  \\
        & CVaR-$0.1$ & 473.84  $\pm$ 0.10 &   \\
        & Episode Length & 500.00  $\pm$ 0.00 &   \\
       \bottomrule
        \end{tabular}
        % \vspace{-1mm}
    \end{table*}

==> sections/results-ablated-medium.tex <==
\begin{table*}[t]
    \centering
    \caption { \label{table:offline-ablated-medium}}
\begin{tabular}{@{}ccccccc@{}}
        \toprule
        &  \textbf{Algorithm}  & \textbf{\alg}-0.1  \\ \midrule
        \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\small{half}}}} 
        & Expected Value & -51.56  $\pm$ 0.25 \\
        & CVaR-$0.1$ & -54.91  $\pm$ 0.93 \\
        %  & Steps & 200    &  200   &  200   &  200   \\
        \midrule
       \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{walker}}}} 
        & Expected Value & 91.66  $\pm$ 8.87 & \\
        & CVaR-$0.1$ & 54.70  $\pm$ 1.98  \\
        & Episode Length & 199.81  $\pm$ 6.49     \\
        \midrule
        \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\small{hopper}}}} 
        & Expected Value & 112.81  $\pm$ 4.64 &  \\
        & CVaR-$0.1$ & 71.28  $\pm$ 23.21   \\
        & Episode Length & 146.08  $\pm$ 4.01   \\
       \bottomrule
        \end{tabular}
        % \vspace{-1mm}
    \end{table*}

==> sections/results-mujoco-expert.tex <==
\begin{table*}[htpb]
    \centering
    \caption{Performance on offline MuJoCo data sets with expert (E) environments. 
    In the first block, we show O-RAAC optimized for CVaR 0.1, WCPG for CVaR 0.1, O-D4PG (risk-neutral) and RAAC (designed for off-policy RL). 
    In the second block we show \alg optimizing the $\alpha$=0.25-quantile ($\text{\alg}_{\text{CVaR}_{0.25}}$), \alg optimizing the CPW risk distortion ($\text{\alg}_{\text{CPW}}$), BEAR (offline risk-neutral) and the behavioral policy (Imitation learning IL-VAE).
    In all environments, \alg has a higher CVaR than benchmarks. 
    In environments that terminate, \alg has a longer duration too. 
    Finally, \alg also has better or equivalent risk-neutral performance than benchmarks. 
    As an ablation, RAAC performs poorly in the offline setting.
    \label{table:offline-expert}}

\begin{tabular}{@{}ccccccc@{}}
    \toprule
    Env &  Criterion  & \textbf{\alg} & O-WCPG & O-D4PG & RAAC  \\ \midrule
    \ \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-E}}}} 
    &$\text{CVaR}_{0.1}$  Returns & \textbf{595.3  $\pm$ 191.0} & 248.4  $\pm$ 232.3 & \textbf{555.8  $\pm$ 263.2} & 2.74 $\pm$ 12.8 \\
    & Average  Returns & \textbf{1180.4  $\pm$ 77.8}  &  \textbf{905.0  $\pm$ 107.2}  & \textbf{1099.8  $\pm$ 152.7}  & 29.8 $\pm$ 3.0 \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-E}}}} 
      & $\text{CVaR}_{0.1}$  Returns& \textbf{1171.8  $\pm$ 71.3} & 361.8  $\pm$ 32.5 & 772.5  $\pm$ 54.7 & 53.9  $\pm$ 2.0 \\
    & Episode Duration & \textbf{431.8  $\pm$ 11.0} & 301.4  $\pm$ 31.1 & 405.4  $\pm$ 12.2 &  195.5  $\pm$ 6.1 \\
    & Average  Returns & \textbf{2005.8  $\pm$ 56.4} & 1372.4  $\pm$ 160.1 & 1869.9  $\pm$ 62.8 & 82.9  $\pm$ 6.4 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-E}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{979.5  $\pm$ 27.7} & 720.0  $\pm$ 33.8 & 606.4  $\pm$ 31.4 & 473.84 $\pm$ 0.1 \\
    & Episode Duration & \textbf{463.5  $\pm$ 6.5} & 301.2  $\pm$ 0.6 & 267.7  $\pm$ 2.5 &  \textbf{500 $\pm$ 0} \\
    & Average  Returns & \textbf{1384.5  $\pm$ 33.11} & 897.6  $\pm$ 12.1 & 783.1  $\pm$ 18.2 & 474.75 $\pm$ 0.1 \\
    \midrule 
    
    
    \toprule
          &    & $\textbf{\alg}_{\text{CVaR}_{0.25}}$ & $\textbf{\alg}_{\text{CPW}}$ & BEAR & IL-VAE  \\ \midrule
    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-E}}}} 
    &$\text{CVaR}_{0.1}$  Returns & \textbf{694.8  $\pm$ 34.3} & 357.9  $\pm$ 66.5 & 43.9 $\pm$ 19.6   & 259.6 $\pm$ 83.5\\
    & Average  Returns & \textbf{1184.7 $\pm$ 7.3}  &  974.4  $\pm$ 21.1 & 556.9  $\pm$ 15.4   & 754.3 $\pm$ 18.13 \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-E}}}} 
      & $\text{CVaR}_{0.1}$  Returns& 669.6  $\pm$ 133.1 & 818.5  $\pm$ 89.4 & 1016.6  $\pm$ 48.6 & 344.9 $\pm$ 301.5 \\
    & Episode Duration & \textbf{436.2 $\pm$ 7.3} & \textbf{454.3  $\pm$ 7.9} & \textbf{462.8  $\pm$ 4.5} & \textbf{348.3 $\pm$ 130.0}  \\
    & Average  Returns & 1757.9 $\pm$ 48.1 & 1874.2  $\pm$ 34.3 & 1782.5  $\pm$ 31.5 & 1217.3 $\pm$ 179.5 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-E}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{729.5 $\pm$ 128.5} & 487.6  $\pm$ 0.6 & 851.7  $\pm$ 30.4 & 773.7 $\pm$ 36.2 \\
    & Episode Duration & 433.9 $\pm$ 6.3 & 159.7  $\pm$ 0.1 & 430.8  $\pm$ 4.2 & \textbf{498.1 $\pm$ 1.2}  \\
    & Average  Returns & 1303.6 $\pm$ 21.2 & 495.9  $\pm$ 0.3  & 1180  $\pm$ 11.7 & 1116.4 $\pm$ 13.1 \\
   \bottomrule
    \end{tabular}
    % \vspace{-1mm}
\end{table*}







% \begin{table*}[t]
%     \centering
%     \caption{Performance of  \alg compared to other benchmarks (O-WCPG, O-D4PG, BCQ) on offline MuJoCo data sets with expert (E) environments. We also show performance of the behavioral policy (Dataset), performance of \alg optimizing the $\alpha$=0.25-quantile ($\text{\alg}_{\text{CVaR}_{0.25}}$), performance of \alg optimizing another risk distortion, namely the cumulative probability weighting function ($\text{\alg}_{\text{CPW}}$) and performance of the ablated \alg (without the VAE component).
%     In all environments, \alg has a higher CVaR than benchmarks. 
%     In environments that terminate, \alg has a longer duration too. 
%     Finally, \alg also has better or equivalent risk-neutral performance than benchmarks. 
%     As an ablation, RAAC performs poorly in the offline setting.
%     When not specified results reported are when optimizing for the $\alpha$=0.1-quantile.
%     \label{table:offline-expert}}

% \begin{tabular}{@{}ccccccc@{}}
%     \toprule
%     Env &  Criterion  & \textbf{\alg} & O-WCPG & O-D4PG & RAAC  \\ \midrule
%     \ \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-E}}}} 
%     &$\text{CVaR}_{0.1}$  Returns & \textbf{595.3  $\pm$ 191.0} & 248.4  $\pm$ 232.3 & \textbf{555.8  $\pm$ 263.2} & 2.74 $\pm$ 12.8 \\
%     & Average  Returns & \textbf{1180.4  $\pm$ 77.8}  &  \textbf{905.0  $\pm$ 107.2}  & \textbf{1099.8  $\pm$ 152.7}  & 29.8 $\pm$ 3.0 \\
%     \midrule
%    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-E}}}} 
%       & $\text{CVaR}_{0.1}$  Returns& \textbf{1171.8  $\pm$ 71.3} & 361.8  $\pm$ 32.5 & 772.5  $\pm$ 54.7 & 53.9  $\pm$ 2.0 \\
%     & Episode Duration & \textbf{431.8  $\pm$ 11.0} & 301.4  $\pm$ 31.1 & \textbf{405.4  $\pm$ 12.2} &  195.5  $\pm$ 6.1 \\
%     & Average  Returns & \textbf{2005.8  $\pm$ 56.4} & 1372.4  $\pm$ 160.1 & 1869.9  $\pm$ 62.8 & 82.9  $\pm$ 6.4 \\
%     \midrule
%     \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-E}}}} 
%     & $\text{CVaR}_{0.1}$  Returns & \textbf{979.5  $\pm$ 27.7} & 720.0  $\pm$ 33.8 & 606.4  $\pm$ 31.4 & 473.84 $\pm$ 0.1 \\
%     & Episode Duration & \textbf{463.5  $\pm$ 6.5} & 301.2  $\pm$ 0.6 & 267.7  $\pm$ 2.5 &  500 $\pm$ 0 \\
%     & Average  Returns & \textbf{1384.5  $\pm$ 33.11} & 897.6  $\pm$ 12.1 & 783.1  $\pm$ 18.2 & 474.75 $\pm$ 0.1 \\
%     \midrule 
    
    
%     \toprule
%           &    & $\textbf{\alg}_{\text{CVaR}_{0.25}}$ & $\textbf{\alg}_{\text{CPW}}$ & BEAR/BCQ & Dataset  \\ \midrule
%     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-E}}}} 
%     &$\text{CVaR}_{0.1}$  Returns & \textbf{483.5  $\pm$ 217.9} & 325.5  $\pm$ 143.7 & 951.9  $\pm$ 148.6 & 1158.5 $\pm$ 27.8 \\
%     & Average  Returns & \textbf{1114.9 $\pm$ 139.2}  &  1022.4  $\pm$ 45.6  & 1478.9  $\pm$ 32.7   & 1782.5 $\pm$ 7.3 \\
%     \midrule
%    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-E}}}} 
%       & $\text{CVaR}_{0.1}$  Returns& \textbf{815.0  $\pm$ 140.1} & 968.8  $\pm$ 75.9 & 2027.4  $\pm$ 78.3 & 1674.9 $\pm$ 25.3 \\
%     & Episode Duration & \textbf{437.4 $\pm$ 9.3} & 451.8  $\pm$ 8.62 & 496.1  $\pm$ 2.15 &   \\
%     & Average  Returns & \textbf{1867.7 $\pm$ 62.9} & 2006.3  $\pm$ 51.2 & 2317.0  $\pm$ 14.3 & 2200.7 $\pm$  6.7 \\
%     \midrule
%     \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-E}}}} 
%     & $\text{CVaR}_{0.1}$  Returns & \textbf{1073.0 $\pm$ 33.5} & 487.8  $\pm$ 0.3 & 1644.1  $\pm$ 15.6 & 1616.1 $\pm$  3.1 \\
%     & Episode Duration & \textbf{443.3 $\pm$ 8.9} & 159.9  $\pm$ 0.15 & 494.4  $\pm$ 0.72 &   \\
%     & Average  Returns & \textbf{1384.3 $\pm$ 21.4} & 496.2  $\pm$ 0.5  & 1760.6  $\pm$ 3.8 & 1774.3 $\pm$  1.7 \\
%    \bottomrule
%     \end{tabular}
%     % \vspace{-1mm}
% \end{table*}

==> sections/results-mujoco-medium.tex <==
\begin{table*}[htpb]
    \centering
    \caption{Performance on offline MuJoCo datasets with with medium (M) environments. In the first block, we show O-RAAC optimized for CVaR 0.1, WCPG for CVaR 0.1, O-D4PG (risk-neutral) and RAAC (designed for off-policy RL). 
    In the second block we show \alg optimizing the $\alpha$=0.25-quantile ($\text{\alg}_{\text{CVaR}_{0.25}}$), \alg optimizing the CPW risk distortion ($\text{\alg}_{\text{CPW}}$), BEAR (offline risk-neutral) and the behavioral policy (Imitation learning IL-VAE).
    In all environments, \alg has a higher CVaR than benchmarks. 
    In environments that terminate, \alg has a longer duration too. 
    Finally, \alg also has better or equivalent risk-neutral performance than benchmarks. 
    As an ablation, RAAC performs poorly in the offline setting.
    \label{table:offline-medium}}
\begin{tabular}{@{}ccccccc@{}}
    \toprule
    Env &  Criterion  & \textbf{\alg} & O-WCPG & O-D4PG & RAAC  \\ \midrule
    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{214.1 $\pm$ 35.9}  & 75.9 $\pm$ 14.3  & 66.0 $\pm$ 34.4 & -54.9  $\pm$ 0.9 \\
    & Average  Returns  & \textbf{330.6 $\pm$ 30.4}  & \textbf{316.1 $\pm$ 23.3}  & \textbf{340.6 $\pm$ 20.0}  & -51.6  $\pm$ 0.3 \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{750.5  $\pm$ 153.5} & -15.0  $\pm$ 40.7 & 30.6  $\pm$ 28.8 & 54.7  $\pm$ 2.0  \\
    & Episode Duration &  397.4  $\pm$ 18.5  & 184.9  $\pm$ 12.1 & 248.8  $\pm$ 8.9 & 199.8  $\pm$ 6.5 \\
    & Average  Returns  & \textbf{1282.4  $\pm$ 19.3} & 283.3  $\pm$ 36.7 & 307.7  $\pm$ 19.9 & 91.7  $\pm$ 8.9 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & \textbf{1416.1  $\pm$ 28.1} & -87.1  $\pm$ 24.5 & 1007.5  $\pm$ 28.2 & 71.3  $\pm$ 23.2 \\
    & Episode Duration &  \textbf{499.3  $\pm$ 1.2} & 99.3  $\pm$ 0.1 & 358.3  $\pm$ 3.1 & 146.1  $\pm$ 4.0\\
    & Average  Returns  & 1482.2  $\pm$ 4.3 & 68.5  $\pm$ 7.6 & 1098.0  $\pm$ 10.6 & 112.8  $\pm$ 4.6\\
    \midrule 
    

    \toprule
          &    & $\textbf{\alg}_{\text{CVaR}_{0.25}}$ & $\textbf{\alg}_{\text{CPW}}$ & BEAR & IL-VAE  \\ \midrule
    \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-M}}}} 
    &$\text{CVaR}_{0.1}$  Returns & \textbf{252.1  $\pm$ 13.8} & \textbf{253.0  $\pm$ 8.7} & 15.2 $\pm$ 30.1  & 10.2 $\pm$ 22.9 \\
    & Average  Returns & \textbf{316.6  $\pm$ 5.1}  &  \textbf{318.3  $\pm$ 2.9}  & \textbf{312.3  $\pm$ 19.8}  & \textbf{354.3 $\pm$ 9.21} \\
    \midrule
   \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-M}}}} 
      & $\text{CVaR}_{0.1}$  Returns& 497.3  $\pm$ 71.2 & 500.8  $\pm$ 71.0 & 517.1  $\pm$ 66.2 & -83.8 $\pm$ 20.9 \\
    & Episode Duration & \textbf{478.9  $\pm$ 5.7} & \textbf{477.2  $\pm$ 2.6} &  \textbf{468.3  $\pm$ 7.6} & 245.7 $\pm$ 9.0  \\
    & Average  Returns & \textbf{1257.4 $\pm$ 27.1} & \textbf{1304.3  $\pm$ 15.8} & \textbf{1317.5  $\pm$ 31.3} & 425.3 $\pm$ 36.7 \\
    \midrule
    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-M}}}} 
    & $\text{CVaR}_{0.1}$  Returns & 1107.5  $\pm$ 13.9 & 968.5  $\pm$ 8.6 & 1252.3  $\pm$ 46.7 & 726.9 $\pm$ 39.0 \\
    & Episode Duration & 418.9  $\pm$ 5.8 & 373.3  $\pm$ 1.8 & 481.2  $\pm$ 2.2 & 461.9 $\pm$ 3.7  \\

    & Average  Returns & 1336.8  $\pm$ 21.0 & 1188.0  $\pm$ 6.3 & \textbf{1574.8  $\pm$ 7.9} & 1081.0 $\pm$ 16.5 \\
   \bottomrule
    \end{tabular}
    % \vspace{-1mm}
\end{table*}

% \begin{table*}[t]
%     \centering
%     \caption{Performance of  \alg compared to other benchmarks (O-WCPG, O-D4PG, BCQ) on offline MuJoCo data sets with medium (M) environments. We also show performance of the behavioral policy (Dataset), performance of \alg optimizing the $\alpha$=0.25-quantile ($\text{\alg}_{\text{CVaR}_{0.25}}$), performance of \alg optimizing another risk distortion, namely the cumulative probability weighting function ($\text{\alg}_{\text{CPW}}$) and performance of the ablated \alg (without the VAE component).
%     In all environments, \alg has a higher CVaR than benchmarks. 
%     In environments that terminate, \alg has a longer duration too. 
%     Finally, \alg also has better or equivalent risk-neutral performance than benchmarks. 
%     As an ablation, RAAC performs poorly in the offline setting.
%     When not specified results reported are when optimizing for the $\alpha$=0.1-quantile.
%     \label{table:offline-medium}}
% \begin{tabular}{@{}ccccccc@{}}
%     \toprule
%     Env &  Criterion  & \textbf{\alg} & O-WCPG & O-D4PG & RAAC  \\ \midrule
%     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-M}}}} 
%     & $\text{CVaR}_{0.1}$  Returns & \textbf{214.1 $\pm$ 35.9}  & 75.9 $\pm$ 14.3  & 66.0 $\pm$ 34.4 & -54.9  $\pm$ 0.9 \\
%     & Average  Returns  & \textbf{330.6 $\pm$ 30.4}  & \textbf{316.1 $\pm$ 23.3}  & \textbf{340.6 $\pm$ 20.0}  & -51.6  $\pm$ 0.3 \\
%     \midrule
%    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-M}}}} 
%     & $\text{CVaR}_{0.1}$  Returns & \textbf{750.5  $\pm$ 153.5} & -15.0  $\pm$ 40.7 & 30.6  $\pm$ 28.8 & 54.7  $\pm$ 2.0  \\
%     & Episode Duration &  \textbf{397.4  $\pm$ 18.5}  & 184.9  $\pm$ 12.1 & 248.8  $\pm$ 8.9 & 199.8  $\pm$ 6.5 \\
%     & Average  Returns  & \textbf{1282.4  $\pm$ 19.3} & 283.3  $\pm$ 36.7 & 307.7  $\pm$ 19.9 & 91.7  $\pm$ 8.9 \\
%     \midrule
%     \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-M}}}} 
%     & $\text{CVaR}_{0.1}$  Returns & \textbf{1416.1  $\pm$ 28.1} & -87.1  $\pm$ 24.5 & 1007.5  $\pm$ 28.2 & 71.3  $\pm$ 23.2 \\
%     & Episode Duration &  \textbf{499.3  $\pm$ 1.2} & 99.3  $\pm$ 0.1 & 358.3  $\pm$ 3.1 & 146.1  $\pm$ 4.0\\
%     & Average  Returns  & \textbf{1482.2  $\pm$ 4.3} & 68.5  $\pm$ 7.6 & 1098.0  $\pm$ 10.6 & 112.8  $\pm$ 4.6\\
%     \midrule 
    

%     \toprule
%           &    & $\textbf{\alg}_{\text{CVaR}_{0.25}}$ & $\textbf{\alg}_{\text{CPW}}$ & BEAR/BCQ & Dataset  \\ \midrule
%     \multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{half-M}}}} 
%     &$\text{CVaR}_{0.1}$  Returns & \textbf{223.1  $\pm$ 44.8} & 255.8  $\pm$ 9.1 & 9.9 $\pm$ 45.8 & 9.3 $\pm$ 5.9 \\
%     & Average  Returns & \textbf{321.2  $\pm$ 17.0}  &  319.6  $\pm$ 2.8  & 348.9  $\pm$ 28.4  & 344.6 $\pm$ 6.0 \\
%     \midrule
%    \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{walker-M}}}} 
%       & $\text{CVaR}_{0.1}$  Returns& \textbf{405.5  $\pm$ 118.4} & 590.0  $\pm$ 100.7 & 336.2  $\pm$ 63.7 & 338.1 $\pm$ 5.9 \\
%     & Episode Duration & \textbf{456.1  $\pm$ 15.1} & 457.6  $\pm$ 6.39 &  461.0  $\pm$ 7.21 &   \\
%     & Average  Returns & \textbf{1261.7  $\pm$ 65.7} & 1321.2  $\pm$ 25.8 & 1425.5  $\pm$ 46.3 & 917.6 $\pm$ 6.0 \\
%     \midrule
%     \multirow{3}{*}{\STAB{\rotatebox[origin=c]{90}{\scriptsize{hopper-M}}}} 
%     & $\text{CVaR}_{0.1}$  Returns & \textbf{1085.7  $\pm$ 18.8} & 973.4  $\pm$ 6.2 & 1229.2  $\pm$ 24.8 & 1097.3 $\pm$ 7.2 \\
%     & Episode Duration & \textbf{404.0  $\pm$ 7.1} & 375.9  $\pm$ 3.28 & 490.6  $\pm$ 3.03 &   \\

%     & Average  Returns & \textbf{1293.7  $\pm$ 24.5} & 1196.8  $\pm$ 11.6 & 1433.5  $\pm$ 10.4 & 1356.5 $\pm$ 1.5 \\
%    \bottomrule
%     \end{tabular}
%     % \vspace{-1mm}
% \end{table*}

==> sections/results-mujoco-v2-long.tex <==
%!TEX root=../iclr2021_conference.tex

\begin{table*}[htpb]
    \centering
    \caption{Performance on offline MuJoCo data sets with expert (E) environments. 
    In the first block, we show O-RAAC optimized for CVaR 0.1, WCPG for CVaR 0.1, O-D4PG (risk-neutral) and RAAC (designed for off-policy RL). 
    In the second block we show \alg optimizing the $\alpha$=0.25-quantile ($\text{\alg}_{\text{CVaR}_{0.25}}$), \alg optimizing the CPW risk distortion ($\text{\alg}_{\text{CPW}}$), BEAR (offline risk-neutral) and the behavioral policy (Imitation learning IL-VAE).
    In all environments, \alg has a higher CVaR than benchmarks. 
    In environments that terminate, \alg has a longer duration too. 
    Finally, \alg also has better or equivalent risk-neutral performance than benchmarks. 
    As an ablation, RAAC performs poorly in the offline setting.
    \label{table:offline-long}
    }

\begin{tabular}{@{}ll|ccc|ccc@{}}
    \toprule 
    & \multirow{2}{*}{Algorithm} & & Medium & & & Expert &  \\ 
    & & $\text{CVaR}_{0.1}$ & Mean Return & Duration & $\text{CVaR}_{0.1}$ & Mean Return & Duration \\ 
    \midrule 
    \multirow{8}{*}{\STAB{\rotatebox[origin=c]{90}{Half-Cheetah}}} &
    $\textbf{\alg}_{0.1}$ & \textbf{214.1 (35.9)} & \textbf{330.6 (30.4)} & 200 (0) & \textbf{595.3  (191.0)} & \textbf{1180.4  (77.8)}& 200 (0)\\ 
    & $\textbf{\alg}_{0.25}$ & \textbf{252.1  (13.8)} & \textbf{316.6  (5.1)} & 200 (0) & \textbf{694.8  (34.3)} & \textbf{1184.7 (7.3)} & 200 (0)\\ 
    & $\textbf{\alg}_{\text{CPW}}$ & \textbf{253.0  (8.7)} & \textbf{318.3  (2.9)} & 200 (0) & 357.9  (66.5) & 974.4  (21.1) & 200 (0)\\ 
    & O-WCPG & 75.9 (14.3) & \textbf{316.1 (23.3)} & 200 (0) & 248.4  (232.3) & \textbf{905.0  (107.2)} & 200 (0)\\ 
    & O-D4PG & 66.0 (34.4) & \textbf{340.6 (20.0)} & 200 (0) & \textbf{555.8  (263.2)} & \textbf{1099.8  (152.7)}& 200 (0)\\ 
    & BEAR & 15.2 (30.1) & \textbf{312.3  (19.8)} & 200 (0) & 43.9 (19.6) & 556.9  (15.4) & 200 (0)\\ 
    & RAAC & -54.9  (0.9) & -51.6  (0.3) & 200 (0) & 2.74 (12.8) & 29.8 (3.0) &  200 (0)\\ 
    & VAE & 10.2 (22.9) & \textbf{354.3 (9.21)}& 200 (0) & 259.6 (83.5) & 754.3 (18.13)& 200 (0)\\ 
    & Dataset & 9.3 (5.9) & 344.6 (2.0) & - & 100.4 (7.5) & 727.3 (3.5) & - \\ 
    \midrule
    \multirow{8}{*}{\STAB{\rotatebox[origin=c]{90}{Walker-2D}}} &
    $\textbf{\alg}_{0.1}$ & \textbf{750.5  (153.5)} & \textbf{1282.4  (19.3)} & 397.4  (18.5) & \textbf{1171.8  (71.3)} & \textbf{2005.8  (56.4)} & \textbf{431.8  (11.0)} \\ 
    & $\textbf{\alg}_{0.25}$ & 497.3  (71.2) & \textbf{1257.4 (27.1)} & \textbf{478.9  (5.7)} & 669.6  (133.1) & 1757.9 (48.1) & \textbf{436.2 (7.3)} \\ 
    & $\textbf{\alg}_{\text{CPW}}$ & 500.8  (71.0) & \textbf{1304.3  (15.8)} & \textbf{477.2  (2.6)} & 818.5  (89.4) & 1874.2  (34.3) & \textbf{454.3  (7.9)} \\ 
    & O-WCPG & -15.0  (40.7) & 283.3  (36.7) & 184.9  (12.1) & 361.8  (32.5) & 1372.4  (160.1) & 301.4  (31.1) \\ 
    & O-D4PG & 30.6  (28.8) & 307.7  (19.9) & 248.8  (8.9) & 772.5  (54.7) & 1869.9  (62.8) & 405.4  (12.2) \\ 
    & BEAR & 517.1  (66.2) & \textbf{1317.5  (31.3)} & \textbf{468.3  (7.6)} & 1016.6  (48.6) & 1782.5  (31.5)& \textbf{462.8  (4.5)} \\ 
    & RAAC & 54.7  (2.0) & 91.7  (8.9)& 199.8  (6.5) & 53.9  (2.0)& 82.9  (6.4)& 195.5  (6.1)\\ 
    & VAE & -83.8 (20.9) & 425.3 (36.7) & 245.7 (9.0) & 344.9 (301.5) & 1217.3 (179.5) & \textbf{348.3 (130.0)} \\
    & Dataset& -55.7 (9.4) & 726.6 (16.2) & - & 1028.1 (33.7) & 1894.1 (7.7) &- \\ 
    \midrule 
    \multirow{8}{*}{\STAB{\rotatebox[origin=c]{90}{Hopper-2D}}} &
    $\textbf{\alg}_{0.1}$ & \textbf{1416.1  (28.1)} & 1482.2  (4.3) & \textbf{499.3  (1.2)} & \textbf{979.5  (27.7)} & \textbf{1384.5  (33.11)}&  \textbf{463.5  (6.5)} \\ 
    & $\textbf{\alg}_{0.25}$ & 1107.5  (13.9) & 1336.8  (21.0) & 418.9  (5.8) & \textbf{729.5 (128.5)} & 1303.6 (21.2) & 433.9 (6.3)\\ 
    & $\textbf{\alg}_{\text{CPW}}$ & 968.5  (8.6) & 1188.0  (6.3) & 373.3  (1.8) & 487.6  (0.6) & 495.9  (0.3)& 159.7  (0.1) \\ 
    & O-WCPG & -87.1  (24.5) & 68.5  (7.6) & 99.3  (0.1) & 720.0  (33.8) & 897.6  (12.1)& 301.2  (0.6) \\ 
    & O-D4PG & 1007.5  (28.2) & 1098.0  (10.6) & 358.3  (3.1) & 606.4  (31.4)& 783.1  (18.2)& 267.7  (2.5)\\ 
    & BEAR & 1252.3  (46.7) & \textbf{1574.8  (7.9)} & 481.2  (2.2) & 851.7  (30.4) & 1180  (11.7) & 430.8  (4)\\ 
    & RAAC & 71.3  (23.2) & 112.8  (4.6) & 146.1  (4.0)  & 473.84 (0.1) & 474.75 (0.1)& \textbf{500 (0)}\\ 
    & VAE & 726.9 (39.0) & 1081.0 (16.5) & 461.9 (3.7) & 773.7 (36.2) & 1116.4 (13.1)& \textbf{498 (1)} \\ 
    & Dataset & 674.4 (5.0) & 1068.4 (4.3) & - & 826.8 (11.6) & 1211.4 (2.5) & - \\  
    \bottomrule
\end{tabular}
\end{table*}



